Asymptotically Optimal Belief Space Planning in Discrete Partially-Observable Domains

Robots often have to operate in discrete partially observable worlds, where the states of world are only observable at runtime. To react to different world states, robots need contingencies. However, computing contingencies is costly and often non-optimal. To address this problem, we develop the improved path tree optimization (PTO) method. PTO computes motion contingencies by constructing a tree of motion paths in belief space. This is achieved by constructing a graph of configurations, then adding observation edges to extend the graph to belief space. Afterwards, we use a dynamic programming step to extract the path tree. PTO extends prior work by adding a camera-based state sampler to improve the search for observation points. We also add support to non-euclidean state spaces, provide an implementation in the open motion planning library (OMPL), and evaluate PTO on four realistic scenarios with a virtual camera in up to 10-dimensional state spaces. We compare PTO with a default and with the new camera-based state sampler. The results indicate that the camera-based state sampler improves success rates in 3 out of 4 scenarios while having a significant lower memory footprint. This makes PTO an important contribution to advance the state-of-the-art for discrete belief space planning.

==> bilder/algorithms/random_graph.tex <==

\begin{algorithm}[h!]
\caption{Random Graph Creation}\label{alg:random}
\KwData{$q_{start}$, $W$, $maxIterations$}
\KwResult{$G_{random}$}
    $G_{random}$.init($q_{start}$)\;
    $iteration = 0$\;
    \While{$iteration < maxIterations$}{
        $sampledWorldIdx$ = random.uniformInt(0, $W$.getnumWorlds())\;
        $W$.setState($sampledWorldIdx$)\;
        $randomValue$ = random.uniform(0, 1)\;
        \eIf{$randomValue$ < 0.2}{
            $randomState$ = sampler.sampleGoal()\;
        }{
            $randomState$ = sampler.sampleUniform()\;
        }
        \If{!isValid($randomState$,  $W$)}{
            continue\;
        }
        $v$ = addVertex($G_{random}$)\;
        $v$.state = $randomState$\;
        $v$.observableObjects = targetsFound($randomState$, $W$)\;
        \For{$worldIdx$ = 0; $worldIdx$ < $W$.getnumWorlds(); $worldIdx$++}{
            $W$.setState($worldIdx$)\;
            $nearestStates$ = getNearestStatesInRadius($v$, $W$, radius=0.5)\;
            \For{$u$ in $nearestStates$}{
                \If{isMotionValid($v$, $u$, $W$)}{
                    \eIf{!edgeExists($v$, $u$, $G_{random}$)}{
                        e = addEdge($v$, $u$, $G_{random}$)\;
                    }{
                        e = getEdge($v$, $u$, $G_{random}$)\;
                    }
                    e.validWorlds.push\_back($worldIdx$)\;
                }
            }
        }
        $iteration$++\;
    }
\end{algorithm}


==> deprecated/deprecated_camera_sampler.tex <==

%\begin{table}[t]
%\centering
%\begin{tabular}{lc}
%\toprule
%Argument & Explanation \\
%$bounds$ & list containing the boundaries of values that a sampled state can take \\
%\hline
%$W$ & the world object \\
%\hline
%$objectPositions$ & list of the positions of all partially observable objects \\
%\hline
%$baseO\!f\!f\!set$ & the desired height of the camera in the sampled state \\
%\hline
%$robotId$ & id of the robot \\
%\hline
%$cameraLinkId$ & id of the link that corresponds to the camera of the robot \\
%\bottomrule
%\end{tabular}
%\caption{Attributes of the camera-based state sampler class.}
%\label{tab:cam}
%\end{table}

%Inverse kinematics is used to calculate the configuration of the remaining joints of the robot so that the target object can be seen by the camera. This method can compute a state in configuration space in which the end effector of the robot is at a desired position in the world space. Thus, to calculate the joint values using inverse kinematics, the desired position and orientation of the camera are required. For simplifying the calculation of the inverse kinematics, the desired position of the camera link is set to the origin (line 9). The height of the camera, i.e. its value on the z-axis, is set to the $baseO\!f\!f\!set$ argument that is specified at the initialization of the sampler. E.g., this could be the z-position of the camera at the start configuration of the robot. Next, also the desired orientation needs to be computed (lines 12 - 20). For this, the viewing direction has to be calculated which accounts for the difference between the sampled base position and the origin position that is used for solving the inverse kinematics problem (line 12). The direction needs to be normalized (line 13). Then, a rotation matrix that specifies the orientation of the camera link is computed (lines 14 - 19). The first column of the matrix corresponds to the normalized cross-product of the direction and the unit vector that points in the positive z direction. The second column consists of the normalized cross-product of the direction and the first row of the matrix. The last column is the normalized direction. This matrix is then transformed to its quaternion representation by using the function \textsc{toQuaternion}.

==> deprecated/deprecated_evaluation.tex <==
\section{Evaluation\label{sec:evaluation}}

This section is concerned with the implementation details of the PTO planner. It introduces four experiments that are used to evaluate the planner. Furthermore, the asymptotic optimality of the planner is discussed empirically, and the computation times of single parts of the algorithm are analyzed.

\section{Open Motion Planning Library}
In contrast to the method introduced by Phiquepal et al., \cite{pathtree}, in this thesis, the PTO planner is implemented as an extension for the Open Motion Planning Library (OMPL)\cite{ompl}, a widely-used, open-source motion planning framework implemented in C++. It is a collection of multiple state-of-the-art sampling-based motion planning algorithms. Moreover, it provides several different state spaces and state samplers that can be used to solve motion planning problems. However, OMPL itself has no visualization capabilities and must be integrated into a system that provides the simulation of robots and environments, as well as important functions such as collision checking.

\section{PyBullet Simulator}
In order to validate the PTO planner, a simulator with visualization capabilities is needed. We use the Python-based PyBullet simulator \cite{pybullet}, which can access the OMPL library by using Python bindings. It enables the creation and visualization of complex 3-D environments and the detection of collisions between objects. Furthermore, it has the capability to use virtual cameras. This is essential for detecting partially observable objects in the environment. Also, inverse kinematics can be computed, which is inevitable for the camera state sampler (see section \ref{sec:camera_sampler}). PyBullet also comes with several debug options. For example, it is possible to execute the planned path tree with all possible paths in parallel while also visualizing the paths, states with observation points, and start- and goal states.\\

The following experiments are implemented in Python building on a simple OMPL to PyBullet interface \cite{interface} that uses the OMPL Python bindings.
 
\section{Primitive Planner Functions in PyBullet}
To use PyBullet, we must define the primitive functions from section \ref{sec:setup}. It is possible to import complete environments, objects, and robots to PyBullet. For the path tree creation, it is important to define the objects that are only partially observable explicitly. While all other objects in our experiment appear in a grayish color, they are displayed colorfully. This simplifies the recognition of the objects by the camera.\\

As described in section \ref{sec:setup}, the functions \textsc{isValid} and \textsc{targetsFound} need to be defined in the context of the simulator. They are being called during the sampling process that is handled by OMPL. We can use the collision checking capabilities of PyBullet to define the \textsc{isValid} function. Given a state and the world, the function first requests the current state of the world. Then, it checks for collisions of permanent obstacles, as well as collisions of partially observable objects with the robot.\\

For the function \textsc{targetsFound}, we need to define a virtual camera using PyBullet. The camera is attached to a specific link of the robot. \textsc{targetsFound} also depends on the state the robot is set to and in which it queries the camera image. The function also depends on the world. E.g., in a world in which all partially observable objects are present, the robot might not see one object because it is occluded by another one. Still, there might exist a world in which this occluding object does not exist, and thus the robot can observe the object behind. Because of this, the function also updates the viewable objects in the simulated world.\\

In the image processing itself, any detection method can be used. Since object detection is not in the scope of the thesis, the problem is simplified by choosing distinct colors for the partially observable objects. Because of this, \textsc{targetsFound} can analyze whether a color corresponding to an object appears in the image. 
It can then translate the color to the corresponding id of the object. The function returns a list of all object ids that the robot's camera can see at the given state.\\

We can also define the camera-based state sampler introduced in section \ref{sec:camera_sampler} using Python. It can use the inverse kinematic solver that is included in PyBullet. Joint values can be computed which lead to a given pose of the camera. The sampler inherits from the OMPL real vector state sampler. Additionally, it adds a method to sample a good camera position. This method can be called by the PTO planner during the generation of the rapidly exploring random graph.


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/envs/sar.png}
    \caption{Search and rescue environment: The Franka robot arm \cite{franka} is mounted on the iRobot Create 2 mobile base \cite{irobot}. The end effector of the robot has a camera attached to it. The task is to rescue a dog \cite{dog} that can be located at four different places in the shown office space. The partially observable locations are represented by differently colored dogs. The office is self-designed, but it uses objects from \cite{office}. The robot should start in the configuration that is shown in image a. There are four different goal configurations, one for each possible position of the dog. In all goal configurations, the robot holds the dog with its end effector. Exemplary, the goal state that corresponds to the red dog location is shown in image b. The PTO planner is concerned with planning a path tree towards all four goal states. The resulting path tree is displayed in both images a and b. Segments of the path that are the same for multiple belief states are shown using black lines. All other segments correspond to final beliefs and thus can be associated with a certain location. These segments are colored so that they match the dog they correspond to. The observation points of the path tree are also visualized as colored dots in the image. The colors of the dots illustrate which potential dog location can be observed from this state.}
    \label{fig:env_sar}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/envs/sar-belief.png}
    \caption{Path tree of the search and rescue environment from Figure \ref{fig:env_sar} that is computed when using the initial belief $b=(0.33, 0.33, 0.33, 0.01)$. The small probability corresponds to the world in which the dog is at the purple location.}
    \label{fig:env_sar_b}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/envs/parking_3x2_edited.png}
    \caption{Parking environment: A car (from \cite{car}) with an attached camera should park at an empty parking lot. The start position of the car is the origin marked with the axis lines. Two parking lots are directly in front of the car, while two more are around a corner. All combinations of existent cars are possible, excluding the world in which all parking lots are occupied. A path tree planned by PTO is visualized in images a - e. For reasons of visibility, the path tree is not displayed in one single image. Instead, each image shows the path that follows the path tree to exactly one leaf node. All leaf nodes correspond to a certain belief. This belief is visualized by making the cars transparent to a specific level. If a car is definitely not existing in the belief, it is fully transparent and the other way around. If the car exists in 50 percent of the worlds that are compatible with the belief, the transparency of the car is also set to 50 percent. The observation points of the path tree are also visualized as colored dots in the image. The colors of the dots illustrate which parking lot can be observed from this state.}
    \label{fig:env_parking}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/benchmarks/door_0-3000-50-12.png}
    \caption{Solution cost and success rate of the door environment \ref{fig:env_door} depending on the number of iterations. The graphs are generated using 12 runs of the PTO planner with different seeds. The x-axis of both graphs represents the number of sampling iterations of the random graph creation. The solution cost stands for the average costs of the planned path trees of the 12 runs. The corresponding standard deviation is also visualized. The success rate is given in percent and specifies how many of the 12 runs managed to find a solution. The cost and the success rate are both shown for 12 runs using the default, uniform state sampler compared to 12 runs that use the camera-based state sampler introduced in section \ref{sec:camera_sampler}. A planner that uses the camera-based state sampler takes approximately 1229 seconds to complete 3000 iterations. For the same number of iterations, a planner that uses uniform sampling takes approximately 1596 seconds.}
    \label{fig:bench_door}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/benchmarks/sar_0-6000-100-12.png}
    \caption{Solution cost and success rate of the search and rescue environment \ref{fig:env_sar} depending on the number of iterations. The graphs are generated using 12 runs of the PTO planner with different seeds. The x-axis of both graphs represents the number of sampling iterations of the random graph creation. The solution cost stands for the average costs of the planned path trees of the 12 runs. The corresponding standard deviation is also visualized. The success rate is given in percent and specifies how many of the 12 runs managed to find a solution. The cost and the success rate are both shown for 12 runs using the default, uniform state sampler compared to 12 runs that use the camera-based state sampler introduced in section \ref{sec:camera_sampler}. A planner that uses the camera-based state sampler takes approximately 1781 seconds to complete 6000 iterations. For the same number of iterations, a planner that uses uniform sampling takes approximately 591 seconds.}
    \label{fig:bench_sar}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/benchmarks/obs_0-4000-50-12.png}
    \caption{Solution cost and success rate of the warehouse environment \ref{fig:env_obs} depending on the number of iterations. The graphs are generated using 12 runs of the PTO planner with different seeds. The x-axis of both graphs represents the number of sampling iterations of the random graph creation. The solution cost stands for the average costs of the planned path trees of the 12 runs. The corresponding standard deviation is also visualized. The success rate is given in percent and specifies how many of the 12 runs managed to find a solution. The cost and the success rate are both shown for 12 runs using the default, uniform state sampler compared to 12 runs that use the camera-based state sampler introduced in section \ref{sec:camera_sampler}. A planner that uses the camera-based state sampler takes approximately 459 seconds to complete 4000 iterations. For the same number of iterations, a planner that uses uniform sampling takes approximately 195 seconds.}
    \label{fig:bench_obs}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/benchmarks/parking_0-3000-50-12.png}
    \caption{Solution cost and success rate of the parking environment \ref{fig:env_parking} depending on the number of iterations. The graphs are generated using 12 runs of the PTO planner with different seeds. The x-axis of both graphs represents the number of sampling iterations of the random graph creation. The solution cost stands for the average costs of the planned path trees of the 12 runs. The corresponding standard deviation is also visualized. The success rate is given in percent and specifies how many of the 12 runs managed to find a solution. The cost and the success rate are both shown for 12 runs using the default, uniform state sampler compared to 12 runs that use the camera-based state sampler introduced in section \ref{sec:camera_sampler}. A planner that uses the camera-based state sampler takes approximately 324 seconds to complete 3000 iterations. For the same number of iterations, a planner that uses uniform sampling takes approximately 347 seconds.}
    \label{fig:bench_parking}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/benchmarks/toy_0-1000-50-12.png}
    \caption{Solution cost and success rate of the toy environment \ref{fig:env_parking} depending on the number of iterations. The graphs are generated using 12 runs of the PTO planner with different seeds. The x-axis of both graphs represents the number of sampling iterations of the random graph creation. The solution cost stands for the average costs of the planned path trees of the 12 runs. The corresponding standard deviation is also visualized. The success rate is given in percent and specifies how many of the 12 runs managed to find a solution. The cost and the success rate are both shown for 12 runs using the default, uniform state sampler compared to 12 runs that use the camera-based state sampler introduced in section \ref{sec:camera_sampler}.}
    \label{fig:bench_toy}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/envs/obs_edited.png}
    \caption{Warehouse environment: As in the search and rescue experiment, the Franka  robot arm \cite{franka} is mounted on the iRobot Create 2 mobile base \cite{irobot}. The end effector of the robot has a camera attached to it. The objective is to retrieve an item from the shown warehouse (from \cite{warehouse}). The partially observable object can be in exactly two different positions which are represented by the red and the blue box on the shelves (from \cite{shelf}). The special feature of this environment is the small window in the wall that allows the robot to see the items directly without entering the area behind the wall. The start state of the robot is marked with a black dot. The PTO planner computes a path tree towards both items which is also visualized in the image. Shared segments of the tree are shown using black lines, while the two colored lines represent segments that correspond to the final beliefs that match the color of the item. In the shown configuration of the robot, it observes the blue item which leads to the branching of the tree.}
    \label{fig:env_obs}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/envs/toy_final.png}
    \caption{Environment used to demonstrate asymptotic optimality: The iRobot create 2 \cite{irobot} should find a path from the start state on the left side towards the goal state on the right side. Both states are represented by black dots. The red and green obstacles are only partially observable. The non-simplified path tree planned by the PTO planner is depicted using black lines. Observation points are represented by dots in the color that matches the observed object.}
    \label{fig:env_toy}
\end{figure}


\section{Asymptotic Optimality}
The asymptotic optimality of PTO has been discussed in section \ref{sec:optiomality}. It is also supported empirically by the benchmark results of the simple experiment shown in Figure \ref{fig:env_toy}. The iRobot Create 2 robot should find a path tree towards a goal state, but there might be two partially observable obstacles in the way.

The benchmark results can be seen in Figure \ref{fig:bench_toy}. For both PTO planners that use a uniform state sampler and for planners that use the camera-based sampler, the solution cost converges after around 400 iterations and does not improve further. The standard deviation approaches zero for all cases. This provides evidence that the optimal solution has been found. Exemplary, the computed non-simplified path of one planner is shown in Figure \ref{fig:env_toy}.


==> deprecated/deprecated_pto.tex <==
\section{Discrete Partially-Observable Belief Space Planning\label{sec:methods}}

A belief space planning problem is defined by its world space $W = (\X, \H)$, and its belief space $\B$ which consists of
\begin{itemize}
    \item $x\in \X$: the state of the robot in its $n$-dimensional state space $\X$,
    \item $s \in \H$: the state of the world from a finite, discrete set of possible world hypotheses $\H$. %Each entry of $s$ stands for an object, while $0$ symbolizes non-existing objects and $1$ represents existing objects.
    \item $b \in \B$: a probability distribution over the world hypothesis space $\H$ with $\B$ being the set of all probability distributions on $\H$
\end{itemize}

We distinguish between two main world states. 
The first type of states are partially observable obstacles, where an object can, at run time, be in a certain number of possible states. 
An example is a door which could be open (0) or closed (1). 
Figure \ref{fig:simple_door} shows an example with a red and a blue door, where we have four distinct world hypotheses as
\begin{align}
    \H_{door} = \{(0, 0),
    (1, 0),
    (0, 1),
    (1, 1)\},
\end{align}
with a world state $(i,j)$ referring to the states of the red and the blue door. 

The second type of world states are partially observable goals.
A partially observable goal refers to a goal region which can have different states at runtime.
An example is an object we want to pick up, but which can exist at different locations. 
Figure \ref{fig:simple_goals} shows a box that can be at three different locations in a warehouse, creating three distinct world hypotheses, which are:
\begin{align}
    \H_{box} = \{(1, 0, 0),
    (0, 1, 0),
    (0, 0, 1)\}
\end{align}
where a world state indicates where an object is to be found.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/simple_door.png}
    \caption{Environment that consists of two partially observable doors, represented with red and blue colors. The robots represent different sampled states. The robot starts at the black state and needs to plan a path to the goal state represented by the white flag. The field of view of the robot's camera is shaded gray in front of the robot. In the red state, the robot is able to observe the state of the red door, and in the blue state, it can observe the state of the blue door. Depending on the observations, the path branches at these observation points.}
    \label{fig:simple_door}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{bilder/worlds.png}
%    \caption{World hypotheses of the environment shown in Figure \ref{fig:simple_door}. Each of the two doors can either exist or not exist which results in four different possible states of the world.}
%    \label{fig:worlds}
%\end{figure}

\label{sec:pogoals}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/simple_goals.png}
    \caption{Environment that consists of three partially observable goal states, represented with a red, green, and blue box. The robots represent different sampled states. The robot starts at the black state and needs to plan a path to the goal states. The field of view of the robot's camera is shaded gray in front of the robot. At the red state, the robot is able to observe the state of the red box, and at the green state, it can observe the state of the green box. Depending on the observations, the path branches at these observation points.}
    \label{fig:simple_goals}
\end{figure}
%

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{bilder/worlds_gaols.png}
%    \caption{World hypotheses of the environment shown in Figure \ref{fig:simple_goals}. Exactly one of the partially observable goals must exist in all possible world states. Since there are three different goals, there are three possible world states.}
%    \label{fig:worlds_goals}
%\end{figure}

\subsection{Path Tree}
\label{sec:pathtree}
Each state can be associated with a belief $b\in\mathcal{B}$. $b$ is a probability distribution over all possible world hypotheses and $\mathcal{B}$ is the set of all possible probability distributions given an initial belief state. When the robot observes an object, it knows about the object's state with certainty such that the following applies: $p(o \mid x, s) \in\{0.0,1.0\}, x \in \mathbb{X}^n, \forall s \in \mathcal{H}, \forall o \in\mathcal{O}$, with $\mathbb{X}$ being the configuration space and $\mathcal{O}$ being the space of all possible observations. As a result, the number of belief states is finite which is a required property for our algorithm. Our goal is to plan a path tree over these belief states. The root node of the path tree is the starting state of the robot that is associated with an initial belief state $b$. Whenever the robot is located at a state where it can observe a partially observable object that has not been seen yet, the belief state gets updated and the path tree branches into two paths that correspond to the new belief states. At planning time, the robot does not know in which world hypothesis it is. Hence, it does not know about the information it will receive at observation points and thus the path tree needs to have a plan for both possible observations. However, at execution time, the word is in a specific state. Thus, at every observation point, there is only one possible observation and only one successor of the current belief state. \\

Belief states are updated as follows: From a specific observation $o\in\mathcal{O}$ follows that only a subset of all possible world states $\mathcal{H}$ is valid depending on the value of the observation.\\

This can be illustrated using the following example: If the red door is observed in the example from Figure \ref{fig:worlds}, only the world states $1$ and $3$ are valid if the door is open, and the states $2$ and $4$ if the door is closed. Equation \ref{eq:belief_update} shows the belief update with the initial belief $b=(0.25, 0.25, 0.25, 0.25)$. In this belief state, all four worlds depicted in Figure \ref{fig:worlds} are equally probable. After the observation, either the world $1$ and $3$ or $2$ and $4$ are equally probable.

\begin{equation}
\label{eq:belief_update}
    \boxed{\begin{aligned} 
      (0.25, 0.25, 0.25, 0.25)
    \end{aligned}} \xrightarrow{\text{observation of the red door}}
    \boxed{\begin{aligned}
     (0.5, 0, 0.5, 0)\\ 
     (0, 0.5, 0, 0.5)
    \end{aligned}}
\end{equation}

For the world hypotheses $\mathcal{H}_{door}$ and $\mathcal{H}_{box}$, the corresponding belief states when starting in the evenly distributed initial beliefs $b_{door}^{init}=\{0.25, 0.25, 0.25, 0.25\}$ and $b_{box}^{init}=\{0.33, 0.33, 0.33\}$ would be:\\

\begin{center}
\begin{minipage}{0.4\linewidth}
\begin{align}
\begin{split}
    \mathcal{B}_{door} =\: &\{\{0.25, 0.25, 0.25, 0.25\},\\
    &\{0.5, 0.5, 0, 0\},\\
    &\{1, 0, 0, 0\},\\
    &\{0, 1, 0, 0\},\\
    &\{0, 0, 0.5, 0.5\},\\
    &\{0, 0, 1, 0\},\\
    &\{0, 0, 0, 1\},\\
    &\{0.5, 0, 0.5, 0\},\\
    &\{0, 0.5, 0, 0.5\}\}
\end{split}
\end{align}
\end{minipage}
\hspace{1cm}
\begin{minipage}{0.4\linewidth}
\begin{align}
\begin{split}
    \mathcal{B}_{box} =\: &\{\{0.33, 0.33, 0.33\},\\
    &\{1, 0, 0\},\\
    &\{0, 0.5, 0.5\},\\
    &\{0, 1, 0\},\\
    &\{0, 0, 1\},\\
    &\{0.5, 0, 0.5\},\\
    &\{0.5, 0.5, 0\}\}
\end{split}
\end{align}
\end{minipage}
\end{center}

We consider a path tree to be complete if all of its leaf nodes fulfill the goal condition. This does not necessarily mean that all partially observable objects need to be observed during the execution of the path-tree. Rather, a path tree that does not branch at all but finds a path to the goal state is also considered complete. This also requires that there is a solution for all possible states of the world.

\subsection{Optimization Objective}
Analogous to the paper by Phiquepal et al. \cite{pathtree}, the optimization objective is constructed as follows:

\begin{subequations}
\begin{align}
& \psi^*=\underset{\psi}{\operatorname{argmin}} \sum_{(u, v) \in \psi} C(u, v) p\left(v \mid \psi, b_0\right), \label{eq:objective}\\
& \text { s.t. } \nonumber\\
& \forall s \in \mathcal{H} \exists l \in \mathcal{L}(\psi) \mid G(l), \label{eq:complete}\\
& \mathcal{V}(u, v), \forall(u, v) \in \psi, \label{eq:valid}\\
& b_v(s)=\frac{p(o \mid s) b_u(s)}{\sum_{s^{\prime}} p\left(o \mid s^{\prime}\right) b_u\left(s^{\prime}\right)}, \forall s \in \mathcal{H}, \forall(u, o, v) \in \psi\label{eq:update}
\end{align}
\end{subequations}

whereby $C(u, v)$ is the cost of the edge that connects the nodes $u$ and $v$. The objective defined by the equation \ref{eq:objective} is to find an optimal path tree $\psi^*$ that minimizes the sum of the costs $C(u, v)$ over all pairs of nodes in a path tree $\psi$, while also taking into account the conditional probability of reaching the node $v$ given an initial belief $b_0$. 
Also, some constraints apply: Constraint \ref{eq:complete} makes sure that for each state $s\in\mathcal{H}$, it must exist at least one leaf node $l\in\mathcal{L}(\psi)$ that satisfies the goal condition given by $G(l)$. $\mathcal{L}(\psi)$ gives the set of all leaf nodes of the path tree $\psi$. This condition ensures the completeness of the path tree. Furthermore, the constraint \ref{eq:valid} checks if all edges $(u, v)\in\psi$ are valid as given by $\mathcal{V}(u, v)$. The constraint \ref{eq:update} specifies that the belief state $b_v(s)$ of the node $v$ should be consistent with the belief $b_u(s)$ of its parent node $u$ when making the observation $o$ while transitioning from $u$ to $v$. $p(o|s)$ is the observation model.

\section{Path Tree Optimization}

\label{sec:algorithm}
This chapter is concerned with the development of the PTO planner to construct a path tree. Since the planning process of the PTO planner is done step-wise, it can be split up into multiple subsections. First, the world object is introduced as a crucial part of planning in belief space. Afterwards, the algorithms that make up the planner are explained in detail. Each of the individual algorithms only creates intermediate representations of the final path tree. Hence, the return value of one algorithm is used by the following one until the complete path tree is built. The planning process consists of the following algorithms:\\

\begin{figure*}[h]
    \centering
        \begin{tikzpicture}[node distance=0.1*\columnwidth, >=latex, thick, box/.style={draw, rectangle, text width=0.1*\columnwidth, minimum height=0.1*\columnwidth, align=center}]
            \node[box] (A) {Random Graph Creation};
            \node[box, right = of A] (B) {Belief Graph Creation};
            
        \end{tikzpicture}
    \caption{Structure of the PTO algorithm. The respective algorithm parts are explained in sections \ref{sec:create_random}, \ref{sec:create_belief_graph}, \ref{sec:compute_costs}, and \ref{sec:create_path}.}
    \label{fig:order_algs}
\end{figure*}

\subsection{Primitive Planner Functions}
\label{sec:setup}
In this section, we define several primitive functions necessary for planning. First, a world object must be initialized. The world object is essential for planning in belief space. It stores all the possible world hypotheses, including the current state of the world. Also, it keeps track of all possible belief states. It is initialized with the number of partially observable objects and an initial belief. Also, a flag indicates whether the partially observable objects are obstacles or goal states. During construction, the world object creates a list of all possible world hypotheses. Analogous to sections \ref{sec:poobstacles} and \ref{sec:pogoals}, either all combinations of different states of all partially observable objects or only combinations in which exactly one object exists are added to that list.\\

Furthermore, the world object provides methods used to create a path tree. They are explained in detail the first time they are used in one of the following algorithms. An overview with short explanations can be found in Table \ref{tab:world_methods}.\\

\begin{table}[htbp]
\caption{Methods of the world object.}
\begin{center}
\begin{tabular}{|c|c|}
\hline
\textsc{getNumWorlds} & returns the number of distinct\\
 & world hypotheses \\
\hline
\textsc{setState} & sets the world to the state that\\
 & corresponds to the given index \\
\hline
\textsc{getAllBeliefStates} & returns a list of all\\
 & reachable belief states in the world \\
\hline
\textsc{getCompatibleBeliefs} & returns a list of beliefs\\
 & that are compatible with the given\\
 & worlds \\
\hline
\textsc{observe} & returns a list containing\\
 & the beliefs that result if the given\\
 & objects are observed at the given belief \\
\hline
\end{tabular}
\label{tab:world_methods}
\end{center}
\end{table}

As a next step, the functions \textsc{isValid} and \textsc{targetsFound} need to be defined.\\

The \textsc{isValid} function takes a state and the world as arguments. Depending on whether the state is valid, e.g. there are no collisions between the robot and objects in the environment, a boolean value is returned. It is important that the world is set to the corresponding world state before calling this function since it also checks for collisions with those partially observable objects that exist in the current state of the world.\\

The \textsc{targetsFound} function takes a state and the world state as arguments. It returns a list of objects found in the camera image at the given configuration given by the state variable. Thereby, the environment of the simulator is set to the given world state. The function analyzes the image and recognizes which partially observable objects are visible. It returns a list containing the indices of the observed objects. The camera is also part of the simulator.\\

Finally, a state sampler must be set that can generate configurations within the configured state space. The state sampler is responsible for the sampling strategy during the creation of the random graph. Hence, it has a major influence on the created random graph and on the final path tree.

\subsection{Random Graph Creation}
\label{sec:create_random}
The PTO planning process starts with creating a so-called rapidly exploring random graph ~\cite{rrtstar}. This process is based on the RRT planner ~\cite{rrt}, and especially on its variant RRG \cite{rrtstar} that is explained in section \ref{sec:rrt}. Analogous to the RRG planner, creating the random graph consists of sampling states in the configuration space of the robot. Nodes of the random graph are associated with the following properties:
\begin{itemize}
    \item a state that describes the configuration of the robot
    \item a list of object indices that represents the partially observable objects that can be seen by the robot at the corresponding state
\end{itemize}
Associated with the edges of the random graph is the following property:
\begin{itemize}
    \item a list containing world indices that stand for the world hypotheses in which the edge is valid
\end{itemize}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/random_graph.png}
    \caption{Sampling process of the rapidly exploring random graph for the example environment introduced in Figure \ref{fig:simple_door}. The black robot symbolizes the start state, while the white flag stands for the goal state of this planning problem. Sampled states are displayed as filled dots. States in which the robot cannot observe any of the partially observable doors are depicted in black. If the robot is able to observe one of the two doors, the corresponding observations are represented with either red or blue dots. The edges of a random graph are only valid in certain worlds, represented with different colors, as stated in the legend.}
    \label{fig:random_graph}
\end{figure}

Algorithm \ref{alg:random} describes the process of the random graph creation, which is also illustrated in Figure \ref{fig:random_graph}. As parameters, the algorithm receives the start configuration of the robot $q_{start}$, the world $W$, and the number of sampling iterations $maxIterations$. First, a new graph is initialized with the starting configuration of the robot, meaning the new graph contains exactly one node that is associated with the start state (line 2). The algorithm runs until $maxIterations$ states have been sampled. Inside the loop, a world state is sampled randomly (line 5), and the world is set to the sampled state (line 6).\\

Afterwards, a sampler that can be configured separately randomly either samples the goal state or uniformly samples a state within the bounds of the configuration space (lines 7 - 12). Now the \textsc{isValid} function is called. If the sampled state is not valid in the sampled world, the algorithm continues with the next execution of the loop and repeats the sampling process (lines 13 - 15). Otherwise, the state is valid and thus a new node is created in the random graph (line 16). The new node is then linked to the sampled state (line 17).\\

Thereafter, the function \textsc{targetsFound} is called (line 18). As explained in section \ref{sec:setup}, it returns a list of object indices corresponding to the partially observable objects that can be seen by the robot's camera at the sampled configuration. This list is also associated with the node in the random graph. In Figure \ref{fig:random_graph}, the sampled states are illustrated using different colored dots. Depending on which objects can be observed at the corresponding states, the dots either have the color of the observed object or they are black if no object can be seen from that configuration.\\

Next, the algorithm iterates over all the possible states of the world (line 19). It then sets the world state to the index of the loop (line 20). Thereafter, the function \textsc{getNearestStatesInRadius} is called (line 21). It uses an internal data structure that stores states for all worlds. Given a state, the world, and a radius, a list of all states that are within the specified radius around the sampled state is returned. The algorithm iterates over those states (line 22) and calls the function \textsc{isMotionValid} (line 23). \textsc{isMotionValid} uses the \textsc{isValid} function to check whether a motion from one state to another is valid in the current world. For this purpose, it densely samples the path and calls \textsc{isValid} on the intermediate states. Only if the motion is valid, the corresponding edge is added to the random graph (lines 24 - 25). If the edge already exists because it was already valid in a world that has been sampled before, it does not get added again. In both cases, the valid worlds property of the edge gets updated by adding the current world index (line 29).\\

Figure \ref{fig:random_graph} also illustrates the added edges. It can be seen that all states that are located within a certain radius of each other are connected by edges. However, these edges have different colors, representing their world validities. The sampling is repeated until the maximum number of iterations is reached. Thereafter, the random Graph is returned.

\begin{algorithm}[h!]
\caption{Random Graph Creation}\label{alg:random}
\KwData{$q_{start}$, $W$, $maxIterations$}
\KwResult{$G_{random}$}
    $G_{random}$.init($q_{start}$)\;
    $iteration = 0$\;
    \While{$iteration < maxIterations$}{
        $sampledWorldIdx$ = random.uniformInt(0, $W$.getnumWorlds())\;
        $W$.setState($sampledWorldIdx$)\;
        $randomValue$ = random.uniform(0, 1)\;
        \eIf{$randomValue$ < 0.2}{
            $randomState$ = sampler.sampleGoal()\;
        }{
            $randomState$ = sampler.sampleUniform()\;
        }
        \If{!isValid($randomState$,  $W$)}{
            continue\;
        }
        $v$ = addVertex($G_{random}$)\;
        $v$.state = $randomState$\;
        $v$.observableObjects = targetsFound($randomState$, $W$)\;
        \For{$worldIdx$ = 0; $worldIdx$ < $W$.getnumWorlds(); $worldIdx$++}{
            $W$.setState($worldIdx$)\;
            $nearestStates$ = getNearestStatesInRadius($v$, $W$, radius=0.5)\;
            \For{$u$ in $nearestStates$}{
                \If{isMotionValid($v$, $u$, $W$)}{
                    \eIf{!edgeExists($v$, $u$, $G_{random}$)}{
                        e = addEdge($v$, $u$, $G_{random}$)\;
                    }{
                        e = getEdge($v$, $u$, $G_{random}$)\;
                    }
                    e.validWorlds.push_back($worldIdx$)\;
                }
            }
        }
        $iteration$++\;
    }
\end{algorithm}

\subsection{Belief Graph Creation}
\label{sec:create_belief_graph}
An essential part of creating the path tree is to translate the sampled random graph to belief space. This is done by creating another graph which is called a belief graph. Similarly to the random graph, nodes of the belief graph are associated with the following properties:
\begin{itemize}
    \item a state
    \item a list containing the indices of observed objects
    \item a belief, as introduced in section \ref{sec:pathtree}
    \item a boolean variable that states whether the vertex fulfills the goal condition
\end{itemize} 
Edges of the belief graph are associated with:
\begin{itemize}
    \item a boolean property that stores whether the edge is a connection between nodes that are connected to the same belief states or not
\end{itemize}

The process of creating a belief graph is described by Algorithm \ref{alg:belief}. The arguments of the algorithms are a random graph $G_{random}$ and the world $W$. First, the belief graph gets initialized (line 2). Then, the algorithm iterates over all vertices of the random graph (line 3) and over all belief states (lines 4 - 12). The function \textsc{isVertexValid} takes a vertex and a belief state as arguments and returns a boolean value whether the vertex is reachable in the given belief state. Thus, it returns false, if the node is not incident with at least one edge that is valid in the given belief state. The function is called for each combination of nodes of the random graph and beliefs (line 5). If the given vertex is reachable in the given belief, a new node is added to the belief graph (line 6). It takes over the state and the list of observable objects from the corresponding random graph node (lines 7 - 8). The node further gets associated with the belief state corresponding to the current iteration (line 9).\\

Also, it stores whether the state is fulfilling the goal condition in the current belief as returned by the function \textsc{isGoal} (line 10). For planning with partially observable obstacles, the goal condition is fulfilled if the sampled state matches the goal state. If we plan a path to partially observable goals, the belief state of the final node must be final. This means that the belief state is certain of being in a particular world, e.g. a belief state $b=(b_1,\ldots,b_n) \in \{0,1\}^n,\: |\{b_i = 1\}_{i\in\{1,\ldots,n\}}| = 1$. This process of creating this first representation of the belief graph is visualized in Figure \ref{fig:belief_graph_1}.\\

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/belief_graph_1.png}
    \caption{Process of transforming a random graph to a belief graph for the example environment introduced in Figure \ref{fig:simple_door}. As a first step, all nodes of the random graph are copied for all beliefs in which the node is incident with at least one edge that is valid in that belief. This can be thought of as adding a new layer of sampled states for all belief states.}
    \label{fig:belief_graph_1}
\end{figure}

After all nodes have been added to the belief graph, edges, that are connecting nodes that are associated with the same belief, are added to the graph (lines 14 - 22). To do so, the algorithm iterates over the edges of the random graph (line 14). It calls the world method \textsc{getCompatibleBeliefs} which takes a list of valid world indices and returns a list of beliefs that are compatible with these indices (line 15). For all of these beliefs (lines 16 - 21), the algorithm adds a new edge to the belief graph (line 19). The function \textsc{getBeliefGraphIdxFromRandomGraphIdx} is used to convert the source and target nodes from the random graph edge to the corresponding vertices of the belief graph (lines 17 - 18). Since at this step the algorithm only adds connections within the same belief, the newly created edge is set not to be a connection between beliefs (line 20). This first process of adding edges to the belief graph is illustrated in Figure \ref{fig:belief_graph_2}.\\

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/belief_graph_2.png}
    \caption{After nodes have been added for all belief states as in Figure \ref{fig:belief_graph_1}, the nodes that are associated with the same belief state are connected with edges according to the random graph.}
    \label{fig:belief_graph_2}
\end{figure}

As the third and last step of creating the belief graph, edges that connect nodes that are associated with observations are added. For this, the algorithm iterates over all vertices that have just been added to the belief graph (line 23). Inside this loop, it iterates over all the objects that can be seen at the state associated with the vertex (line 24). In this loop, it calls the world method \textsc{observe} (line 25). This function takes a belief and a list of object indices as input arguments. It returns a list containing the beliefs that result if the given objects are observed at the given belief as explained in equation \ref{eq:belief_update}.\\

For each of the child belief states (lines 26-32), a new edge is added to the belief graph (line 29). While the source state of the edge is the vertex that corresponds to the iteration of the outer loop, the target state of the edge is computed using helper functions. The function \textsc{getRandomGraphIdxFromBeliefGraphIdx} first translates the source vertex into the corresponding vertex in the random graph (line 27). Afterwards, the function \textsc{getBeliefGraphIdxFromRandomGraphIdx} converts the random graph vertex back to the corresponding vertex in the belief graph with the correct belief (line 28). The edge gets set to be a connection between beliefs (line 30). Furthermore, the target state of the edge gets added to the list of child beliefs that are associated with it (line 31). An exemplary addition of one edge between nodes with different belief states can be seen in Figure \ref{fig:belief_graph_3}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/belief_graph_3.png}
    \caption{Edges are added for nodes that are associated with observations. Following the example from Figure \ref{fig:simple_door}, in the left illustration, the node surrounded by a yellow circle observes the red door. The corresponding state is associated with the belief $(0.25, 0.25, 0.25, 0.25)$. Corresponding to equation \ref{eq:belief_update}, new edges are added to the belief graph. The source of those directed edges is the node that is associated with the observation. The target nodes correspond to the same vertex in the random graph as the source node but they are different vertices in the random graph. They are associated with the beliefs $(0.5, 0, 0.5, 0)$ and $(0, 0.5, 0, 0.5)$ respectively, as follows from equation \ref{eq:belief_update}.}
    \label{fig:belief_graph_3}
\end{figure}

\begin{minipage}{\linewidth}
\begin{lstlisting}[mathescape=true, escapeinside={*}{*}, label={alg:belief}, caption={Belief Graph Creation}]
function createBeliefGraph($G_{random}$, $W$):
    $G_{belief}$.init()
    for ($v$ in getVertices($G_{random}$)) $\{$
        for ($belief$ in $W$.getAllBeliefStates()) $\{$
            if (isVertexValid($v$, $belief$)) $\{$
                $u$ = addVertex($G_{belief}$)
                $u$.state = $v$.state
                $u$.observableObjects = $v$.observableObjects
                $u$.belief = $belief$
                $u$.isGoal = isGoal($u$, $belief$)
            $\}$
        $\}$
    $\}$
    for ($e$ in getEdges($G_{random}$)) $\{$
        $compatibleBeliefs$ = $W$.getCompatibleBeliefs($e$.validWorlds)
        for ($belief$ in $compatibleBeliefs$) $\{$
            $source$ = getBeliefGraphIdxFromRandomGraphIdx($e$.source, $belief$)
            $target$ = getBeliefGraphIdxFromRandomGraphIdx($e$.target, $belief$)
            $e_{belief}$ = addEdge($source$, $target$, $G_{belief}$)
            $e_{belief}$.isWorldConnection = false
        $\}$
    $\}$
    for ($v$ in getVertices($G_{belief}$)) $\{$
        for ($o$ in $G_{belief}$.observableObjects) $\{$
            $newBeliefs$ = $W$.observe($v$.belief, $o$)
            for ($belief$ in $newBeliefs$) $\{$
                $randomGraphIdx$ = getRandomGraphIdxFromBeliefGraphIdx($v$)
                $target$ = getBeliefGraphIdxFromRandomGraphIdx($randomGraphIdx$, $belief$)
                e = addEdge($v$, $target$, $G_{belief}$)
                e.isWorldConnection = true
                $v$.beliefChildren.push_back($target$)
            $\}$
        $\}$
    $\}$
    return $G_{belief}$
\end{lstlisting}
\end{minipage}

\subsection{Computation of the Expected Costs to the Goal}
\label{sec:compute_costs}
Once the belief graph is constructed, we want to calculate the minimized expected costs to the one goal, or to multiple goals for every vertex of the belief graph. The computation is a generalization of Dijkstra's algorithm ~\cite{dijkstra} introduced in section \ref{sec:dijkstra}. It is performing dynamic programming by Bellmann updates. The algorithm is modified to account for graph nodes where an observation is received. Algorithm \ref{alg:costs} describes this process. It receives the belief graph $G_{belief}$ and the world $W$ as arguments. The algorithm uses a priority queue to be able to keep track of what nodes should be updated next, similar to the Dijkstra algorithm. First, the costs for each vertex and the priority queue are initialized (lines 3 - 12). To do this, the algorithm iterates over all vertices of the belief graph (line 5). If the vertex fulfills the goal condition, the costs of this vertex are set to zero and the vertex together with its costs get added to the priority queue. All other vertices are initialized with infinite costs. This is illustrated in Figure \ref{fig:costs_1}.\\

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/costs_1.png}
    \caption{Initialization of the calculation of the costs for a simple environment consisting of only one partially observable obstacle depicted in red. The nodes of the underlying belief graph are visualized. The goal states have a blue outline. Edges between nodes with the same belief state are illustrated in black, while edges between nodes associated with different beliefs are red. Red edges are labeled with the corresponding branching probabilities. In this example, the red obstacle can only be observed at one node which is marked red. Every state is labeled with the costs it is initialized with. Only the goal states have the initial cost of zero, while the costs of all other states are initialized with infinity.}
    \label{fig:costs_1}
\end{figure}

After the initialization process, a loop is executed until the priority queue is empty, meaning there is no more node whose costs can be further optimized (lines 12 - 31). Inside the loop, the algorithm takes the first element of the priority queue, which is the vertex $v$ with the smallest costs (line 13) and it removes this entry from the priority queue (line 14). Using the function \textsc{getAdjacentVertices}, a list consisting of all vertices that are adjacent to $v$ in the belief graph is obtained (line 15). For each neighbor $u$ of $v$ (lines 16 - 30), the algorithm checks if its costs can be improved. If the corresponding edge (line 17) is a connection between nodes with the same beliefs (line 18), the new costs would be the sum of the distance between $u$ and $v$ and the costs of $v$ (line 19). Instead, if the edge corresponds to an observation, the new costs would be the sum of the costs of the children nodes of the corresponding observation multiplied by the probability of the observations (lines 21 - 24). At this point the Algorithm \ref{alg:costs} differs from Dijkstra's algorithm.\\

The branching probability is computed by the world method \textsc{calculateBranchingProbability} (line 23). Given two belief states, it calculates the probability of getting from the parent belief to the child belief as described in Algorithm \ref{alg:branching}. The calculated probability is the sum of the entries of the parent belief state with indices that correspond to positive entries of the child belief state. It follows, that given a uniformly distributed initial belief, the branching probabilities are always $p=0.5$.

\begin{minipage}{\linewidth}
\begin{lstlisting}[mathescape=true, escapeinside={*}{*}, label={alg:branching}, caption={Calculation of Branching Probability}]
double p = 0;
for (int i = 0; i < getNumWorldStates(); i++) {
    if (childBeliefState.at(i) > 0) {
        p += parentBelifState.at(i);
    }
}
\end{lstlisting}
\end{minipage}

If the newly calculated costs are smaller than the previous costs of the vertex $u$, the costs of $u$ get updated and the vertex-costs-pair is added to the priority queue (lines 26 - 29). A visualization of the final state of the algorithm can be seen in Figure \ref{fig:costs_2}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/costs_2.png}
    \caption{After iteratively applying Bellman updates on the nodes of the example from Figure \ref{fig:costs_1}, the resulting minimized expected costs of each node are shown. The final expected cost of this path tree is 17.1.}
    \label{fig:costs_2}
\end{figure}

\begin{minipage}{\linewidth}
\begin{lstlisting}[mathescape=true, escapeinside={*}{*}, label={alg:costs}, caption={Computation of the Expected Costs to the Goal}]
function computeExpectedCostsToGoal($G_{belief}$, $W$):
    $costs$ = []
    $pq$ = PriorityQueue()
    for ($v$ in getVertices($G_{belief}$)) $\{$
        if ($v$.isGoal) $\{$
            $costs$.push_back(0)
            $pq$.push((0, $v$))
        $\}$ else $\{$
            $costs$.push_back($\infty$)
        $\}$
    $\}$
    while (!pq.empty()) $\{$
        $v$ = $pq$.top()
        $pq$.pop()
        $adjacentVertices$ = getAdjacentVertices($v$, $G_{belief}$)
        for ($u$ in $adjacentVertices$) $\{$
            $e$ = getEdge($v$, $u$, $G_{belief}$)
            if (!$e$.isWorldConnection) $\{$
                $newCost$ = calculateDistance($v$, $u$) + costs[$v$]
            $\}$ else $\{$
                $newCost$ = 0
                for ($child$ in $u$.beliefChildren) $\{$
                    $newCost$ += $W$.calculateBranchingProbability($u$.belief, $child$.belief) $*$ $costs$[$child$]
                $\}$                
            $\}$
            if ($newCost$ < costs[$u$]) $\{$
                $costs$[$u$] = $newCost$
                $pq$.push(($newCost$, $u$))
            $\}$
        $\}$
    $\}$
    return costs
\end{lstlisting}
\end{minipage}

\subsection{Path-Tree Creation}
\label{sec:create_path}
After the expected costs are computed, the path tree can be extracted. Nodes in the path tree are associated with the following properties:
\begin{itemize}
    \item a state
    \item a variable that stores if the vertex is fulfilling the goal condition
\end{itemize}
Edges in the path tree store the following property:
\begin{itemize}
    \item a boolean variable stating whether the edge corresponds to a motion or an observation
\end{itemize}
The path tree extraction is done recursively as described in Algorithm \ref{alg:path}. To do so, the recursive algorithm makes use of two member variables of the planner object: the path tree $T$ itself, and a list $pathTreeFinalStates$ that contains all the goal vertices of the path tree (lines 2 - 3). First, $v_{belief}$ is set to the first node of the belief graph $G_{belief}$ (line 5). $v_{belief}$ keeps track of the node of the belief graph that corresponds to the last added node of the path tree. Afterwards, the set $visited$ is initialized (line 6). It is used to store all the nodes of the belief graph that correspond to vertices that have already been added to the path tree. Then, a new vertex $v$ is added to the path tree (line 7). It gets set to the $state$ and $isGoal$ properties of the corresponding belief graph vertex $v_{belief}$.\\

After this initial setup, the function \textsc{createPathTree} is called (line 12). The parameters of the function are the belief graph $G_{belief}$ and the $costs$ as calculated by the previous algorithms \ref{alg:belief} and \ref{alg:costs}. Furthermore, it gets the last node added to the path tree $v$, the corresponding node in the belief graph $v_{belief}$, and the set $visited$. In a while loop (lines 13 - 60), the algorithm first creates a list of all neighbors of the belief graph node $v_{belief}$ (line 14). It tries to find the next best vertex, starting from $v_{belief}$. To do so, $v_{bestVertex}$ is initialized with 0 (line 15). The algorithm iterates over all neighbors $u_{belief}$ of $v_{belief}$ (line 16). If $u_{belief}$ was not yet added to the path tree (line 17), the edge $e$ between $u_{belief}$ and $v_{belief}$ is obtained (line 18). If this edge is related to an observation (line 19), we directly add a new node $v_t$ corresponding to the vertex $v_{belief}$ to the path tree (lines 20 - 22). Also, the corresponding edge between $v$ and $v_t$ is added (line 23). Since it is an observation edge, the \textsc{isWorldConnection} property is set to true (line 24). Because a copy of $u_{belief}$ has been added to the path tree, it gets added to the set of visited vertices (line 25). The algorithm checks if the newly added node $v_t$ is fulfilling the goal condition (line 26). If so, $v_t$ is added to the list $pathTreeFinalStates$. Otherwise, the \textsc{createPathTree} function is recursively called with the new arguments $v_t$ and $u_{belief}$.\\

If the edge $e$ is related to a motion, the algorithm checks if it points to a better node than $v_{bestVertex}$ (lines 31 - 43). Therefore, it calculates the costs corresponding to $u_{belief}$ and $u_{bestVertex}$ by adding together their respective costs and their distance to $v_{belief}$ (lines 32 - 33). If the costs of $u_{belief}$ are smaller than the costs of the current best vertex, or if the best vertex has not yet been updated and thus is zero, the algorithm proceeds with updating $v_{bestVertex}$ (lines 34 - 42). Only if the distance of $v_{belief}$ and $u_{belief}$ is zero, meaning that the base position of the states is the same, $v_{bestVertex}$ is only updated if the already found best vertex does not match the costs of $v_{belief}$ (lines 35 - 39). This makes sure that a perfect next vertex is not overwritten by a node just because the corresponding edge has zero costs.\\

After completing iterating over the neighbor nodes, a new best vertex has been found. This node should be the next vertex in the path tree. Thus, a new node $v_t$ that corresponds to $v_{bestVertex}$ is added to the path tree (lines 46 - 48). If it fulfills the goal condition, it is also added to the set $pathTreeFinalStates$ (lines 50 - 52). Also, the corresponding edge is added with \textit{isWorldConnection} being set to false (lines 53 - 54). The $visited$ set is updated with the added vertex $v_{bestVertex}$ (line 55) and $v$ and $v_{belief}$ are updated to the next states $v_t$ and $v_{bestVertex}$ (lines 56 - 57). If the added vertex fulfills the goal condition, the function terminates (lines 58 - 60). A visualization of the algorithms can be seen in Figure \ref{fig:path_tree}.
  
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/path_tree.png}
    \caption{Extraction of the path tree from the belief graph using the expected costs. We start at the start state that is associated with the initial belief. At each node, we append the best vertex to the tree. At observation nodes, the path tree may branch into two sub-trees. The best node is the vertex that leads to the cost update. The thick green arrows indicate the final path tree.}
    \label{fig:path_tree}
\end{figure}

\begin{minipage}{\linewidth}
\begin{lstlisting}[mathescape=true, escapeinside={*}{*}, label={alg:path}, caption={Path Tree Creation}]
// member variables
$T$.init()
$pathTreeFinalStates$ = $\{\}$

$v_{belief}$ = $G_{belief}$[$0$]
$visited$ = $\{\}$
$v$ = addVertex($T$)
$v$.state = $v_{belief}$.state
$v$.isGoal = $v_{belief}$.isGoal

// recursively construct the path-tree
function createPathTree($G_{belief}$, $costs$, $v$, $v_{belief}$, $visited$):
    while (true) $\{$
        $adjacentVertices$ = getAdjacentVertices($v_{belief}$, $G_{belief}$)
        $v_{bestVertex}$ = 0
        for ($u_{belief}$ in $adjacentVertices$) $\{$
            if ($u_{belief}\notin$ $visited$) $\{$
                $e$ = getEdge($v_{belief}$, $u_{belief}$, $G_{belief}$)
                if ($e$.isWorldConnection) $\{$
                    $v_t$ = addVertex($T$)
                    $v_t$.state = $u_{belief}$.state
                    $v_t$.isGoal = $u_{belief}$.isGoal
                    $e_t$ = addEdge($v$, $v_t$, $T$)
                    $e_t$.isWorldConnection = true
                    $visited$.insert($u_{belief}$)
                    if ($v_t$.isGoal) $\{$
                        $pathTreeFinalStates$.push_back($v_t$)
                    $\}$ else $\{$
                        createPathTree($G_{belief}$, $costs$, $v_t$, $u_{belief}$, $visited$)
                    $\}$
                $\}$ else $\{$
                    $newCosts$ = $costs$[$u_{belief}$] + calculateDistance($v_{belief}$, $u_{belief}$)
                    $oldCosts$ = $costs$[$v_{bestVertex}$] + calculateDistance($v_{belief}$, $v_{bestVertex}$)
                    if ($v_{bestVertex}$ == $0$ or $newCosts$ <= $oldCosts$) $\{$
                        if (calculateDistance($v_{belief}$, $u_{belief}$) == $0$) $\{$
                            if ($oldCosts$ != $costs$[$v_{belief}$] or $bestVertex$ == $0$) $\{$
                                $v_{bestVertex}$ = $u_{belief}$
                            $\}$
                        $\}$ else $\{$
                            $v_{bestVertex}$ = $u_{belief}$
                        $\}$
                    $\}$
                $\}$
            $\}$
        $\}$
        $v_t$ = addVertex($T$)
        $v_t$.state = $v_{bestVertex}$.state
        $v_t$.isGoal = $v_{bestVertex}$.isGoal
        if ($v_t$.isGoal) $\{$
            $pathTreeFinalStates$.push_back($v_t$)
        $\}$
        $e_t$ = addEdge($v$, $v_t$, $T$)
        $e_t$.isWorldConnection = false
        $visited$.insert($v_{bestVertex}$)
        $v$ = $v_t$
        $v_{belief}$ = $v_{bestVertex}$
        if ($v_{bestVertex}$.isGoal) $\{$
            break
        $\}$
    $\}$
\end{lstlisting}
\end{minipage}

\subsection{Path Tree Simplification}
The path tree created by Algorithm \ref{alg:path} is complete, but the planned paths may be unnatural, including many sharp turns. This is due to the nature of the sampling-based approach of creating the random graph as the basis of the PTO planner. Since the PTO algorithm is asymptotically optimal as will be shown in section \ref{sec:optiomality}, the planned path will eventually converge to an optimal solution. Thus, we could increase the number of sampling iterations of the random graph creation. This solution can potentially be very resource-demanding. Instead, in practice, it is advantageous to have a path simplification step. Since the paths can only be simplified between observation points without breaking the core element of the path tree, the path tree needs to be divided into different segments. Each of these segments is then simplified using a shortcutting method to decrease path length. This simplification step is less resource intensive and produces more natural paths.

\section{Asymptotic Optimality}
\label{sec:optiomality}
The case can be made that the proposed algorithm is asymptotically optimal, as defined in section \ref{sec:optimal_planning}.  This means that it is actually able to find the optimal path tree as defined in equation \ref{eq:objective} for an unlimited number of iterations. When the configuration space is sampled densely enough, the created random graph (Algorithm \ref{alg:random}) always contains the optimal solution for all possible world states since RRGs are asymptotically optimal \cite{rrtstar}. This random graph would also contain the path that is found by the RRT$^*$ algorithm ~\cite{rrtstar} which is also asymptotically optimal \cite{optimal}. When expanding the random graph to the belief graph (Algorithm \ref{alg:belief}), the random graph is duplicated for every belief while it only contains nodes and edges that are valid in that belief. Thus, each of these layers of the belief graph still contains the optimal path for the corresponding belief. Since the random graph in this experiment also consists of all possible observation states, the set of edges that connect the observation nodes with corresponding nodes with different beliefs is complete. It follows, that the belief graph contains the optimal solution. Since the optimal solution is extracted with the Dijkstra-like Algorithm \ref{alg:costs}, it can be ensured that the optimal solution is found with enough sampling iterations.

\section{Camera-based State Sampler}
\label{sec:camera_sampler}
The default implementation of the random graph construction from Algorithm \ref{alg:random} samples a random state either uniformly within the bounds of the given state space, or it samples the goal state. With this sampling strategy, it depends on chance whether a partially observable object is seen or not. Since the potential locations of all partially observable objects are known to the planner, we can take advantage of this, by defining our own state sampler which we call the "Camera-based State Sampler". This sampler implements a function that samples configurations in which the robot's camera is directly looking towards a partially observable object that exists in the current world state. An illustration of the behavior of this sampler can be seen in Figure \ref{fig:camera}. It samples a robot configuration in which the robot's camera directly points towards the only partially observable object in the environment. Thus, this object has a high likelihood to be seen by the camera.\\

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bilder/camera2.png}
    \caption{A Franka robot arm \cite{franka} is mounted on the iRobot Create 2 \cite{irobot} mobile base. A camera is attached to the end effector of the arm. In the shown configuration of the robot, its camera points directly to the red object as indicated by the red line of sight. This configuration was sampled using the camera-based state sampler.}
    \label{fig:camera}
\end{figure}

The camera-based state sampler object is initialized with the attributes shown in Table \ref{tab:cam}.\\

\begin{table}
\centering
\begin{tabular}{lcl}
\toprule
Argument & Explanation \\
\specialrule{.1em}{.0em}{.0em}
$bounds$ & list containing the boundaries of values that a sampled state can take \\
\hline
$W$ & the world object \\
\hline
$objectPositions$ & list of the positions of all partially observable objects \\
\hline
$baseO\!f\!f\!set$ & the desired height of the camera in the sampled state \\
\hline
$robotId$ & id of the robot \\
\hline
$cameraLinkId$ & id of the link that corresponds to the camera of the robot \\
\bottomrule
\end{tabular}
\caption{Attributes of the camera-based state sampler class.}
\label{tab:cam}
\end{table}

The class implements the method \textsc{sampleGoodCameraPosition} which is described in Algorithm \ref{alg:cam}. In this thesis, it is applied to mobile manipulators with a two-dimensional base, but the method is generally applicable. It gets an uninitialized state as its argument and it initializes the state with a sampled configuration.\\

First, the algorithm needs to know what object should be seen by the camera. For this purpose, it calls the function \textsc{getExistingObjects} (line 2) that, given the world $W$, returns a list of all partially observable objects that exist in the current world. It then randomly selects one of the objects as the target object, i.e. the object that should be seen by the camera in the configuration that is to be sampled (lines 3 - 4). At first, only the position of the robot's base is sampled. This is done uniformly within the specified bounds of the environment (lines 5 - 6). Then the position of the target object is queried (line 7).\\

Inverse kinematics is used to calculate the configuration of the remaining joints of the robot so that the target object can be seen by the camera. This method can compute a state in configuration space in which the end effector of the robot is at a desired position in the world space. Thus, to calculate the joint values using inverse kinematics, the desired position and orientation of the camera are required. For simplifying the calculation of the inverse kinematics, the desired position of the camera link is set to the origin (line 9). The height of the camera, i.e. its value on the z-axis, is set to the $baseO\!f\!f\!set$ argument that is specified at the initialization of the sampler. E.g., this could be the z-position of the camera at the start configuration of the robot. Next, also the desired orientation needs to be computed (lines 12 - 20). For this, the viewing direction has to be calculated which accounts for the difference between the sampled base position and the origin position that is used for solving the inverse kinematics problem (line 12). The direction needs to be normalized (line 13). Then, a rotation matrix that specifies the orientation of the camera link is computed (lines 14 - 19). The first column of the matrix corresponds to the normalized cross-product of the direction and the unit vector that points in the positive z direction. The second column consists of the normalized cross-product of the direction and the first row of the matrix. The last column is the normalized direction. This matrix is then transformed to its quaternion representation by using the function \textsc{toQuaternion}.\\

To solve the inverse kinematic problem, the \textsc{calculateInverseKinematics} function is used (line 23), which in our case is part of the simulator. It takes the id of the robot and of the camera link, as well as the desired position and quaternion orientation as arguments. Based on these inputs, it computes a joint configuration that leads to the camera pointing towards the target object. The sampled configuration is composed as follows: The first two entries are set to the position of the base (lines 25-26). Then, the remaining state entries are filled with the joint values that were calculated by using inverse kinematics (lines 27 - 31).\\

\begin{minipage}{\linewidth}
\begin{lstlisting}[mathescape=true, escapeinside={*}{*}, label={alg:cam}, caption={Sampling of good camera positions as used by the camera-based state sampler.}]
function sampleGoodCameraPosition($state$):
    $objects$ = getExistingObjects($W$)
    $randomValue$ = random.uniformInt(0, len($objects$))
    $selectedObject$ = $objects$[$randomValue$]
    $basePosition$ = [random.uniform($bounds$[0].low, $bounds$[0].high),
                      random.uniform($bounds$[1].low, $bounds$[1].high)]
    $objectPosition$ = $objectPositions$[$selectedObject$]

    // position of camera link
    $position$ = [0, 0, $baseO\!f\!f\!set$]

    // compute orientation of camera link
    $direction$ = [$objectPosition$[0] - $basePosition$[0], $objectPosition$[1] - $basePosition$[1], 0]
    normalize($direction$)
    $upVector$ = [0, 0, 1]
    $xAxis$ = crossProduct($upVector$, $direction$)
    normalize($xAxis$)
    $yaxis$ = crossProduct($direction$, $xAxis$)
    normalize($yAxis$)
    $matrix$ = transpose($[$xAxis$, $yAxis$, $direction$]$)
    $orientation$ = toQuaternion($matrix$)
    
    $ik$ = culculateInverseKinematics($robotId$, $cameraLinkId$, $position$, $orientation$)

    $state$[0] = $basePosition$[0]
    $state$[1] = $basePosition$[1]
    $i = 0$
    for ($jointPosition$ in $ik$) $\{$
        $state$[2 + i] = $jointPosition$
        $i$ += 1
    $\}$
\end{lstlisting}
\end{minipage}

This camera-based sampler can sample states from which the camera can directly observe partially observable objects. This leads to an increase in states in the random graph that are associated with observations. It can be combined with a uniform sampler to guarantee the asymptotic optimality of the path.\\

The camera-based sampler also implements a method that replaces the uniform sampling of the base position with values that can be passed to the method as arguments. This can be used in the random graph creation described in section \ref{sec:create_random}. Before sampling randomly, new states can be sampled at the corresponding start position of the base while the robot observes the existing objects in this configuration.

==> deprecated/time_analysis.tex <==

\section{Time Analysis}
This section is concerned with the time needed by each part of the PTO algorithm. Table \ref{tab:time} lists the time complexity for each of the discussed algorithm parts. It is noticeable that regardless of the number of sampling iterations, the random graph creation always has the largest contribution to the runtime of the algorithm, with always more than 90 percent. This is mainly due to the validity checking of the sampled states and the corresponding motions. The belief graph creation and the calculation of the expected costs to the goal do not have a significant influence on the runtime of the PTO algorithm. Still, for both algorithms, with more iterations, exponentially more time is needed. The runtime of the belief graph creation depends especially on the number of partially observable objects. With more objects, also the number of reachable belief states grows exponentially, and thus also the size of the belief graph grows comparably quickly. The extraction of the path tree is the second largest contributor to the complete runtime of PTO in the door environment.

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}
\centering
\begin{tabularx}{\linewidth}{|l|Y|Y|Y|Y|Y|}
\hline
Algorithms Part & \multicolumn{5}{c|}{Time per Iterations (in s)} \\
 & 1000 & 1500 & 2000 & 2500 & 3000 \\
\specialrule{.1em}{.0em}{.0em}
Random Graph & $135$ & $289$ & $486$ & $780$ & $1116$ \\
 & ($95.1$\%) & ($92.8$\%) & ($92.4$\%) & ($92.4$\%) & ($92.1$\%) \\
\hline
Belief Graph & $1.70$ & $3.90$ & $6.45$ & $10.74$ & $14.65$ \\
 & ($1.2$\%) & ($1.0$\%) & ($1.2$\%) & ($1.3$\%) & ($1.2$\%) \\
\hline
Costs Calculation & $1.54$ & $4.43$ & $9.78$ & $14.87$ & $24.85$ \\
 & ($1.1$\%) & ($1.4$\%) & ($1.9$\%) & ($1.8$\%) & ($2.0$\%) \\
\hline
Path Tree Extraction & $3.72$ & $13.99$ & $24.05$ & $38.19$ & $56.20$ \\
 & ($2.6$\%) & ($4.5$\%) & ($4.6$\%) & ($4.5$\%) & ($4.6$\%) \\
\hline
\end{tabularx}
\caption{Required time of the PTO planner that uses the camera-based state sampler for different parts of the path tree creation algorithm on the door environment introduced in section \ref{sec:door}. The times are given in seconds and specified for different sampling iterations. The percentage of the total runtime of the algorithm to which they contribute is shown in parentheses.}
\label{tab:time}
\end{table}
